Multi-scale analysis of global electromagnetic instabilities in ITER Pre-Fusion-Power Operation plasmas

Global electromagnetic gyrokinetic simulations are performed with the Particle-in-Cell code ORB5 for an ITER Pre-Fusion-Power-Operation (PFPO) plasma scenario, with half-field (2.65 T) and half-current (7.5 MA). We report on a 'multi-scale' analysis of the discharge, considering eigenmodes and instabilies across three scale-lengths. Although the scenario will nominally have neutral beam heating with particles injected with 1 MeV, Alfv\'en eigenmodes are investigated in the absence of such source, and Reversed Shear (RSAE), Toroidal (TAE) and Elliptical (EAE) Alfv\'en eigenmodes are found with weak damping for moderately low toroidal mode numbers ($10 \leq n \leq 35$). At higher toroidal mode numbers ($40 \leq n \leq 70$), unstable Alfv\'enic modes have been observed close to rational surfaces and are labelled as Beta-induced Alfv\'en eigenmodes (BAE)/Alfv\'enic Ion Temperature Gradient (AITG) modes, since their frequency is associated with the BAE gap and they are driven by the bulk plasma on the Alfv\'enic continuum. These modes are unstable in the absence of energetic particles, and adding a species of energetic particles (with an isotropic 1 MeV slowing down distribution) has negligible impact on their growth rate. At higher toroidal mode numbers ($150 \lessapprox n < 220$), low frequency microscale instabilities are observed.

==> command_DIFF.tex <==
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF


